Towards Real-World Adverse Weather Image Restoration: Enhancing Clearness and Semantics with Vision-Language Models

This paper addresses the limitations of adverse weather image restoration approaches trained on synthetic data when applied to real-world scenarios. We formulate a semi-supervised learning framework employing vision-language models to enhance restoration performance across diverse adverse weather conditions in real-world settings. Our approach involves assessing image clearness and providing semantics using vision-language models on real data, serving as supervision signals for training restoration models. For clearness enhancement, we use real-world data, utilizing a dual-step strategy with pseudo-labels assessed by vision-language models and weather prompt learning. For semantic enhancement, we integrate real-world data by adjusting weather conditions in vision-language model descriptions while preserving semantic meaning. Additionally, we introduce an effective training strategy to bootstrap restoration performance. Our approach achieves superior results in real-world adverse weather image restoration, demonstrated through qualitative and quantitative comparisons with state-of-the-art works.

==> misc/alg.tex <==

\begin{algorithm}[t]
    \caption{Pseudo Label Initialization and Iterative Update}
    \label{alg:training}
    \scriptsize
    \begin{algorithmic}[1]
    \Require VLM-based image assessment function $r^{vlm}$, a set of VLM models $VLMs$, existing image restoration models $Rs$;
    
    \State \textbf{Phase 1: pseudo label initialization}
    \State Initialize $\mathcal{D}^{ps} = \{x_i^u,y_i^{ps}\}_{i=1}^M \gets \emptyset$;
    \For{$x_i^u \in \mathcal{D}^u$, $R \in Rs$}
        % \For{$R \in Rs$}
            \State Get the restoration $\hat{y}_i = R(x_i^u)$;
            \For{each $vlm \in VLMs$} compute $r_i^{vlm}(\hat{y}_i)$;
            \label{algline:vlms-rating}
            \EndFor
            \State Update $y_i^{ps}$ with best $r^{vlm}_i$;
        % \EndFor
    \EndFor

    \State \textbf{Phase 2: iterative update}
    \For{$round = 1 \ to \ n$}
        \State Choose one VLM for $r^{vlm}$;
        \For{$x_i^u \in \mathcal{D}^u$}
            \State Get the restoration $\hat{y}_i = R_{\theta_t}(x_i^u)$ and compute $r_i^{vlm}(\hat{y}_i)$;
            % \State Compute $r^{vlm}$ for pseudo label;
            % \State Compute $r^{vlm}$ for teacher's restoration;
            \State Update $y_i^{ps}$ \textbf{if} better $r^{vlm}_i$;
        \EndFor
        \State Update $\mathcal{D}^{ps}$ using \textcolor{black}{\cref{algline:vlms-rating}} with the predictions of the newly trained model.
        \State Update learned weather prompts $t$ and descriptions $d$.
    \EndFor
    % \Ensure $y = x^n$
    % \State $y \gets 1$
    % \State $X \gets x$
    % \State $N \gets n$
    % \While{$N \neq 0$}
    % \If{$N$ is even}
    %     \State $X \gets X \times X$
    %     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
    % \ElsIf{$N$ is odd}
    %     \State $y \gets y \times X$
    %     \State $N \gets N - 1$
    % \EndIf
    % \EndWhile
    \end{algorithmic}
\end{algorithm}
%\vspace{-5mm}
